Dark matter search in a Beam-Dump eXperiment (BDX) at Jefferson Lab: an update on PR12-16-001

This document is an update to the proposal PR12-16-001 Dark matter search in a Beam-Dump eXperiment (BDX) at Jefferson Lab submitted to JLab-PAC44 in 2016 reporting progress in addressing questions raised regarding the beam-on backgrounds. The concerns are addressed by adopting a new simulation tool, FLUKA, and planning measurements of muon fluxes from the dump with its existing shielding around the dump. First, we have implemented the detailed BDX experimental geometry into a FLUKA simulation, in consultation with experts from the JLab Radiation Control Group. The FLUKA simulation has been compared directly to our GEANT4 simulations and shown to agree in regions of validity. The FLUKA interaction package, with a tuned set of biasing weights, is naturally able to generate reliable particle distributions with very small probabilities and therefore predict rates at the detector location beyond the planned shielding around the beam dump. Second, we have developed a plan to conduct measurements of the muon ux from the Hall-A dump in its current configuration to validate our simulations.

==> BDX-PAC45-upd-opt.tex <==
\section{Background rejection strategies}
\label{sec:opt}
As  reported in Sec.XXX of PR-16-001and confirmed by using FLUKA (see  Sec.~\ref{sec:sim}), the BDX reach is ultimately limited  by  beam-related  neutrinos.
In this Section we describe some analysis procedures to optimize BDX signal-to-background ratio  suggesting strategies for an experimental  measurement  and characterization of the {\it irreducible} background.

\subsection{Neutrino background}
Neutrinos ($\nu_{e}$, $\nu_{\bar e}$,  $\nu_{\mu}$, and   $\nu_{\bar \mu}$) are produced in muon decay and hadronic shower (pion decay). The majority comes from pion and muon decay at rest but a non negligible fraction, due to  in flight pion decay, experience   a significant boost till  several GeV energy.
High energy neutrinos interacting with BDX detector by elastic and inelastic scattering may result in a significant energy deposition ($>$ 500 MeV) that may mimic an em shower produced by the $\chi$-atomic electron interaction.
To estimate the neutrino background we used different simulation tools.   FLUKA has been used to generate neutrinos in 11 GeV electron/dump interaction, propagate them to the BDX location and sample particles  produced in the interaction with the active BDX volume (CsI(Tl)). Reaction products were then feed to GEMC code  that contains a detailed and realistic description of the BDX detector response.
Figure~\ref{neutflux-det} shows the differential energy spectrum of the four neutrino species. Electron neutrinos and anti-neutrinos are suppressed by a factor of hundred wrt $\nu_{\mu}$ and $\bar\nu_{\mu}$. These results are (within a factor of 2) consistent to what obtained using GEMC.
\begin{figure}[h!] 
\center
\includegraphics[width=14.5cm]{figs/neutflux-det.pdf}
\caption{Differential energy spectrum of neutrinos ($\nu_{\mu}$, $\bar\nu_{\mu}$, $\nu_{e}$,  and $\bar\nu_{e}$)  impinging on the  BDX detector volume. {\it  {\color{red}  replace with high stat and better edited figure}}}
\label{fig:neutflux-det}
\end{figure}
FLUKA only considers $\nu$-N and $\bar\nu$-N interactions disregarding  $\nu$-electron and $\bar\nu$-electron interaction.
We checked the validity of this approximation doing an analytical estimate of the $\nu$-e and $\bar\nu$-e contribution finding that for 10$^{22}$ EOT we are expecting less than 1 interaction on the BDX volume.
The $\nu$-Nucleus interaction cross sections used by FLUKA are  reported in Fig.~\ref{neutxsec}.
\begin{figure}[h!] 
\center
\includegraphics[width=12.5cm]{figs/neutxsec.pdf}
\caption{Neutrino-Nucleus interaction cross section for the different species ($\nu_{\mu}$, $\bar\nu_{\mu}$, $\nu_{e}$,  and $\bar\nu_{e}$). {\it  {\color{red}  replace with high stat and better edited figure}}}
\label{fig:neutxsec}
\end{figure}

The implication  to the $\chi$-electron signal measurement for different $\nu$-matter interactions 
 are listed below.
\begin{itemize}
\item{$\nu_\mu$ N $\to \mu $ X: the Charge Current (CC) interaction produces a $\mu$ in the final state (beside the hadronic state X). This reaction can be identified and used to provide an experimental asses of the $\nu_\mu$ background (and therefore estimate the $\nu_e$ contribution) by detecting a $\mu$ scattering in the detector (a MIP signal inside the calorimeter with or w/o activity in IV and OV). Another strategy  would be to exploit the  CC interaction kinematic that favours  $\mu$ emitted  at large angles.}
\item{$\nu_\mu$ N $\to \nu_\mu $ X: the Neutral Current (NC) interaction product is limited to the hadronic state X. This can mimic an em shower if $\pi^0$ ($\gamma$'s) are produced. However, due to the difference in mass, the scattered $\nu$ carries the most part of the available energy providing a small transfer to the hadronic system and reducing the probability of an over-threshold energy deposition.}
\item{$\nu_e$ N $\to \nu_e $ X: same considerations as above.}
\item{$\nu_e$ N $\to e $ X: the CC interaction is the most critical background since it could produce a high energy electron into the detector that mimics the signal.  This background can be rejected considering again the different kinematics of the $\nu$ interaction wrt the  $\chi$-electron scattering. Figure~\ref{neut-ang} shows the comparison of the electron angle (wrt the z axes) for the two reactions.  The significant difference allow to define a selection  cut to identify $\nu_e$ ad separate from the $\chi$.
}
\end{itemize}
\begin{figure}[h!] 
\center
\includegraphics[width=12.5cm]{figs/neutang.pdf}
\caption{Angles of electron produced in $\chi$-electron and  $\nu_e$ N $\to e $ X reactions  . {\it  {\color{red}  replace with high stat and better edited figure}}}
\label{fig:neutxsec}
\end{figure}
We simulated 2.2$10^8$ EOT obtaining, after all rejection cuts and extrapolatation to 10$^{22}$ EOT,  a background of 11 neutrino (3 $\nu_{\mu}$ + 0.2 $\bar\nu_{\mu}$ + 6$\nu_{e}$,  and + 0.7 $\bar\nu_{e}$) . The inventory and the conclusions are in good agreement with estimates obtained with  GEMC simulation reported in PR-16-001
The rejection cuts optimization is in progress. Massive FLUKA simulations will run in the next few months.

\subsection{Off-axes neutrino measurement}
FLUKA and GEMC provide a consistent prediction of the neutrino background in the range of $\sim10$ counts for the whole BDX live time.Thanks to the segmentation of the BDX detector we may experimentally assess the neutrino background by moving the detector off-axes and changing the selection cuts in the analysis. In the previous paragraph we showed that the $\chi$-electron
and the $\nu$-Nucleus interaction have different kinematics (other than different dynamics) that affect the angular distributions in the lab system providing an handle to differentiate the background from the signal.
Assuming a $\chi$-electron maximum number of interaction consistent with the current limit in the parameter space (mainly set by E137 experiment) we proved that moving the BDX detector off-axes by 50 cm would result in 0 signal counts for 10$^{22}$ EOT. This means that BDX detector  will only measure the $\nu$ background. Few off-axes positions (e.g. lateral displacement of  50 cm, 100 cm and 150 cm ) with a set of $\nu$ selection cuts (rather than rejection) in the off-line analysis would allow us  to map out the absolute $\nu$ flux as a function of the off-axes distance and compare to the Monte Carlo simulations. The flux of $\nu_\mu$ will be measured identifying a $\mu^-$ in the BDX detector while the number of $\nu_e$ interactions will be detected  by measuring the back-scattered electron in $\nu_e$ N $\to e $ X.

We are currently optimising the experimental set up and the selection cuts to prove the statistical significance of $\nu$ background characterization. Results obtained so far show than the BDX detector have the capability of measuring neutrinos during the experiment enhancing the experimental sensitivity and providing a solid ground for any positive or negative results.




